Revisiting the Effects of Stochasticity for Hamiltonian Samplers

We revisit the theoretical properties of Hamiltonian stochastic differential equations (SDES) for Bayesian posterior sampling, and we study the two types of errors that arise from numerical SDE simulation: the discretization error and the error due to noisy gradient estimates in the context of data subsampling. Our main result is a novel analysis for the effect of mini-batches through the lens of differential operator splitting, revising previous literature results. The stochastic component of a Hamiltonian SDE is decoupled from the gradient noise, for which we make no normality assumptions. This leads to the identification of a convergence bottleneck: when considering mini-batches, the best achievable error rate is $\mathcal{O}(\eta^2)$, with $\eta$ being the integrator step size. Our theoretical results are supported by an empirical study on a variety of regression and classification tasks for Bayesian neural networks.

==> friction.tex <==


\begin{itemize}
    \item Friction can make the dynamics more robust since it changes the Lipschitz constant
    \item ?Possibly about the time reversibility/detailed balance of the noisy version. Reversible integrators are more robust 
\end{itemize}

{\color{red}POSSIBLE HUGE STEP FORWARD IN EXPLANATION: WE NEED TO DISCUSS THIS}

\begin{itemize}
    \item The relevant biblio is \cite{chen2015convergence},\cite{blanes2008splitting},\cite{leimkuhler2013rational}
    \item I (not found written anywhere in literature...) propose to interpret \hmc as a discretization scheme of the same \sde we are considering above
    \item In particular, by splitting the infinitesimal (Kolmogorov) generator as:
    \begin{equation}
        \mathcal{A}=\text{Pure Hamiltonian}+\text{Pure OU process of the momentum}=\mathcal{H}+\mathcal{D}
    \end{equation}
    Then the integration of the dynamics starting from $\mathbf{z}_0$ for a time $T$ can be expressed as
    \begin{equation}
        \exp{T\mathcal{A}} \mathbf{z}_0=\exp{T\mathcal{D}}\exp{T\mathcal{H}} \mathbf{z}_0+\mathcal{O}(T^2)
    \end{equation}
    where the equality is derived by Taylor expanding the differential operator $\mathcal{A}$+ Baker–Campbell–Hausdorff formula.
    \item Since we split the operator we can solve sequentially the two mappings
    \begin{enumerate}
        \item First we resolve the deterministic Hamiltonian dynamics. This correspond to the inner loop of \hmc algorithm
        \item Then we solve the OU process for momentum. ANALYTICALLY
        \begin{equation}
            \mathbf{r}_T=\exp{-CT}\mathbf{r}_0+\sqrt{2C(1-\exp{-CT})}\mathbf{\nu}
        \end{equation}
        where $\mathbf{r}_0$ is the momentum at the end of the inner loop and $\mathbf{\nu}\sim\mathcal{N}(\mathbf{0},\mathbf{I})$. It is evident that if $CT>>1$ (and this is usually the case since $T$ depends on inner loop duration) a good approximation is
        \begin{equation}
            \mathbf{r}_T=\sqrt{2C}\mathbf{\nu}
        \end{equation}
        a.k.a. momentum resampling!!
    \end{enumerate}
    \item At this point I am fairly confident with the following statement: there is no reason why you shold ever use classical \hmc. Toghether with friction \hmc they are two different discretization schemes of the same \sde but classical \hmc is provably worse.
    
    \item Bonus point for further explanation link on why the \sg noise is asymptotically irrelevant: we can similarly split the full log likelihood into chunks (the minibatches) and use the same theory. IMPORTANT OPEN POINT: CAN WE IMPROVE THE CONVERGENCE RATE BY CONSIDERING THIS PERSPECTIVE? A minibatch is not anymore random but just a split of the full dataset, unbiased BUT "better" than true gradient + memoryless noise
    \item Role of $||\Delta \mathcal{V}_l||$ in \cite{chen2015convergence} paper and non-commutative remainder from Baker–Campbell–Hausdorff?? Is this why you can neglect \sg noise?
\end{itemize}


Hereafter (just to remember) a list of the relevant papers

\begin{itemize}
    \item \cite{suzuki1977convergence} A paper about splitting by Suzuki. The terms f{m,n} are considered. Not practical but "good" to cite
    \item \cite{hatano2005finding} Again by Suzuki. This is useful and higher order Suzuki decomp. are presented (p>1)
    \item \cite{talay1990expansion} A book by Talay. In chapter 2.2. there is the thing about going from local to global (weak error). Good to cite and backup if "my" proof is flawed
    \item \cite{raginsky2017non} Again the book by Raginsky. Hints about time convergence splitting
    \item \cite{leimkuhler2013rational} aper about splitting of diffusion. The hint about hmc being just a split scheme is linked to this (very weakly)
    \item \cite{li2019stochastic} Our NIPS enemy. Luckily not much focus on "stochastic" gradients (only informal mention in appendix E) or splitting interpretation
    \item \cite{rossler2010runge} A reference on Runge Kutta for SDEs
    \item \cite{milstein2013stochastic} Milstein book about numerical sdes. Good again for the local->global error
    \item \cite{mil1986weak} as above, but a paper
    \item \cite{childs2019theory} Trotter and Suzuki decomposition for multi hamiltonian systems. IMPORTANT we use eq. 17 in particular
    \item \cite{childs2019nearly} Splitting Hamiltonian paper
    \item \cite{low2019well} again a paper aobut split Hamilt
\end{itemize}

==> hmc.tex <==
\begin{itemize}
    \item We consider 4 variants of \hmc methods:
    \begin{itemize}
        \item the vanilla \hmc: full gradient and no noise injected or friction 
        \item the naive \sghmc: stochastic gradient and no noise injected or friction 
        \item \sghmc: stochastic gradient with noise injected and friction according to fluctuation dissipation theorem
        \item \hmc with noise injected and friction according to fluctuation dissipation theorem
    \end{itemize}
    The general equation is the following:
    \begin{flalign*}
\begin{cases}
\boldsymbol{d} \thetavect[n]=\eta \boldsymbol{r}[n-1]\\
\boldsymbol{d} \boldsymbol{r}[n]=-\eta\mathbf{C} \boldsymbol{r}[n-1]-\eta( \boldsymbol{g}(\thetavect[n-1]))+\sqrt{\eta}\boldsymbol{w}[n],
\end{cases}
\end{flalign*}
where $\thetavect,\boldsymbol{r}$ are position and momentum respectively, $\boldsymbol{g}(\thetavect)$ is the stochastic gradient (in full gradient settings $\boldsymbol{g}(\thetavect)=\nabla_{\thetavect} U(\thetavect)$ and $w\sim\mathcal{N}(0,2\boldsymbol{C})$ is the injected noise for the versions that use injected noise+friction
    \item We first write the general \fpe for \sde s.
    Generic \sde
    \begin{equation}\label{eq:sde0}
d\zetavect(t)=\boldsymbol{s}(\zetavect(t))dt+\sqrt{2 \boldsymbol{D}(\zetavect(t))}d\boldsymbol{w}(t).
\end{equation}



    \item we write the \sde s for the 4 considered scheme with THE CORRECT $dt$ formalism.
    
    Define the supervariable $\boldsymbol{z}=[\boldsymbol{x},\boldsymbol{r}]^\top$. We can rewrite the system as: 
\begin{flalign*}
\boldsymbol{d}\zetavect[n]= -\eta\begin{bmatrix} \zerovect & -\eye\\ \eye & \boldsymbol{C} \end{bmatrix}\boldsymbol{s}(\zetavect[n-1])+\sqrt{2\eta \boldsymbol{D}}\boldsymbol{\nu}[n]
\end{flalign*}
where $\boldsymbol{s}(\zetavect)=\begin{bmatrix}\boldsymbol g(\thetavect)\\\boldsymbol{M}^{-1}\boldsymbol{r}\end{bmatrix}$, $\boldsymbol{D}(\zetavect)=\begin{bmatrix} \zerovect & \zerovect\\ \zerovect & \boldsymbol{C}\end{bmatrix}$ and $\boldsymbol{\nu}[n]\sim \mathcal{N}(0,\eye)$.\\
Let's assume that $g(\thetavect)=\nabla_{\thetavect} U(\thetavect)+\boldsymbol{k}[n]$, where $\boldsymbol{k}[n]$ is a Gaussian random variable with finite variance $\Bmath$.\\
We substitute $\eta=dt$ and obtain
\begin{equation}
 \boldsymbol{d}\zetavect_t= -\begin{bmatrix} \zerovect & -\eye\\ \eye & \boldsymbol{C} \end{bmatrix} \begin{bmatrix}\nabla_{\thetavect} U(\thetavect_t)\\\boldsymbol{M}^{-1}\boldsymbol{r}_t\end{bmatrix}dt+\sqrt{2 \boldsymbol{D}}\boldsymbol{d\nu}_t
\end{equation}
where $\boldsymbol{d\nu}_t$ is a Brownian motion.\\

\textbf{The key difference with the literature, due to eq. \eqref{eqbuild} is that:}
\begin{equation}
    \eta g(\thetavect)=\eta\nabla_{\thetavect} U(\thetavect)+\eta \boldsymbol{k}[n]\rightarrow \nabla_{\thetavect} U(\thetavect) dt +\sqrt{2 dt \Bmath} \boldsymbol{dw}_t=\nabla_{\thetavect} U(\thetavect) dt+\mathcal{O}(dt^2)
\end{equation}
and since in the \sde only terms up to $\mathcal{O}(dt)$ matters the stochastic gradient noise in the continuous limit becames deterministic \cite{dieuleveut2020bridging}
    \item Contrary to the literature, all 4 methods are provided to converge to the true posterior\begin{itemize}
        \item We study \hmc. In this case $\Cmath=0$
        \item Naive \sghmc = \hmc. This is conceptually truly important. As a trivial consequence \sghmc do converge to the true posterior
        \item \sghmc the matrix $\Cmath $ is user selected and different from zero.
        \item with similar arguments, \hmc with friction is the same as \sghmc. 
    \end{itemize}
    \item \textbf{attention}: in literature someone else is suggesting explicitly that Naive \sghmc is bad: \cite{pmlr-v37-betancourt15}. On the contrary I would argue, by looking at the equations for the bias in trajectory with data resampling within a single trajectory that: if the number of steps per trajectory is a multiple of the number of minibatches, the bias is exactly zero, in any case the field $H$ grows while the error is averaged out. Not clear the comment about not having computational gains.
    \item add some comments on \hmc momentum resampling due to energy conservation and \fpe ss solution w.r.t initial conditions (or alternatively fast variables,...etc...)
\end{itemize}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}


==> order3/explicit_form.tex <==

\begin{equation}
\begin{split}
	\mathbf{r}_1 &= \mathbf{r}_k + \frac{7}{24} \eta \left[-\nabla U(\boldsymbol{\theta}_1) - C \mathbf{M}^{-1} \mathbf{r}_1 \right] \\
	\mathbf{r}_1 + \frac{7}{24} \eta C \mathbf{M}^{-1} \mathbf{r}_1 &= \mathbf{r}_k - \frac{7}{24} \eta \nabla U(\boldsymbol{\theta}_1) \\
	\mathbf{r}_1 &= \frac{\mathbf{r}_k - \frac{7}{24} \eta \nabla U(\boldsymbol{\theta}_1)}{1 + \frac{7}{24} \eta C \mathbf{M}^{-1}}
\end{split}
\end{equation}



\begin{equation}
\begin{split}
	\mathbf{r}_2 &= \mathbf{r}_k + \frac{2}{3} \eta \left[-\nabla U(\boldsymbol{\theta}_1) - C \mathbf{M}^{-1} \mathbf{r}_1 \right]
	+ \frac{3}{8} \eta \left[-\nabla U(\boldsymbol{\theta}_2) - C \mathbf{M}^{-1} \mathbf{r}_2 \right] \\
	%\mathbf{r}_2 + \frac{3}{8} \eta C \mathbf{M}^{-1} \mathbf{r}_2 &= \mathbf{r}_k + \frac{2}{3} \eta \left[-\nabla U(\%boldsymbol{\theta}_1) - C \mathbf{M}^{-1} \mathbf{r}_1 \right]
	%- \frac{3}{8} \eta \nabla U(\boldsymbol{\theta}_2) \\
	\mathbf{r}_2 &= \frac{\mathbf{r}_k + \frac{2}{3} \eta \left[-\nabla U(\boldsymbol{\theta}_1) - C \mathbf{M}^{-1} \mathbf{r}_1 \right]
	- \frac{3}{8} \eta \nabla U(\boldsymbol{\theta}_2)}{1 + \frac{3}{8} \eta C \mathbf{M}^{-1}}
\end{split}
\end{equation}



\begin{equation}
\begin{split}
	\mathbf{r}_3 &= \mathbf{r}_k + \frac{2}{3} \eta \left[-\nabla U(\boldsymbol{\theta}_1) - C \mathbf{M}^{-1} \mathbf{r}_1 \right]
	- \frac{2}{3} \eta \left[-\nabla U(\boldsymbol{\theta}_2) - C \mathbf{M}^{-1} \mathbf{r}_2 \right]
	+ \eta \left[-\nabla U(\boldsymbol{\theta}_3) - C \mathbf{M}^{-1} \mathbf{r}_3 \right] \\
	%
	\mathbf{r}_3 &= \frac{
	\mathbf{r}_k + \frac{2}{3} \eta \left[-\nabla U(\boldsymbol{\theta}_1) - C \mathbf{M}^{-1} \mathbf{r}_1 \right]
	- \frac{2}{3} \eta \left[-\nabla U(\boldsymbol{\theta}_2) - C \mathbf{M}^{-1} \mathbf{r}_2 \right]
	-\eta \nabla U(\boldsymbol{\theta}_3)
	}{1 + \eta C \mathbf{M}^{-1}}
\end{split}
\end{equation}



==> order3/implicit_form.tex <==
We have $h \rightarrow \eta$, so:

\begin{equation}
\begin{split}
	\boldsymbol{\theta}_1 &= \boldsymbol{\theta}_k + \frac{7}{24} \eta \mathbf{M}^{-1} \mathbf{r}_k \\
	\mathbf{r}_1 &= \mathbf{r}_k + \frac{7}{24} \eta \left[-\nabla U(\boldsymbol{\theta}_1) - C \mathbf{M}^{-1} \mathbf{r}_1 \right]
\end{split}
\end{equation}


\begin{equation}
\begin{split}
	\boldsymbol{\theta}_2 &= \boldsymbol{\theta}_k + \frac{25}{24} \eta \mathbf{M}^{-1} \mathbf{r}_k 
	+ \frac{\eta^2}{2} \mathbf{M}^{-1} \left[ -\nabla U(\boldsymbol{\theta}_1) - C \mathbf{M}^{-1} \mathbf{r}_1 \right]
	\\
	\mathbf{r}_2 &= \mathbf{r}_k + \frac{2}{3} \eta \left[-\nabla U(\boldsymbol{\theta}_1) - C \mathbf{M}^{-1} \mathbf{r}_1 \right]
	+ \frac{3}{8} \eta \left[-\nabla U(\boldsymbol{\theta}_2) - C \mathbf{M}^{-1} \mathbf{r}_2 \right]
\end{split}
\end{equation}



\begin{equation}
\begin{split}
	\boldsymbol{\theta}_3 &= \boldsymbol{\theta}_k + \eta \mathbf{M}^{-1} \mathbf{r}_k 
	+ \frac{17}{36} \eta^2 \mathbf{M}^{-1} \left[ -\nabla U(\boldsymbol{\theta}_1) - C \mathbf{M}^{-1} \mathbf{r}_1 \right]
	+ \frac{1}{36} \eta^2 \mathbf{M}^{-1} \left[ -\nabla U(\boldsymbol{\theta}_2) - C \mathbf{M}^{-1} \mathbf{r}_2 \right]
	\\
	%
	\mathbf{r}_3 &= \mathbf{r}_k + \frac{2}{3} \eta \left[-\nabla U(\boldsymbol{\theta}_1) - C \mathbf{M}^{-1} \mathbf{r}_1 \right]
	- \frac{2}{3} \eta \left[-\nabla U(\boldsymbol{\theta}_2) - C \mathbf{M}^{-1} \mathbf{r}_2 \right]
	+ \eta \left[-\nabla U(\boldsymbol{\theta}_3) - C \mathbf{M}^{-1} \mathbf{r}_3 \right]
\end{split}
\end{equation}


\begin{equation}
\begin{split}
	\boldsymbol{\theta}_{k+1} &= \boldsymbol{\theta}_3 + \eta^{3/2} \mathbf{M}^{-1} \sqrt{2C} \left(\mathbf{w}^{(k)}_1/2 + \mathbf{w}^{(k)}_2 \right) \\
	&\quad - C \eta^{5/2} \mathbf{M}^{-2} \sqrt{2C}~\mathbf{w}^{(k)}_1 / 6
\end{split}
\end{equation}


\begin{equation}
\begin{split}
	\mathbf{r}_{k+1} &= \mathbf{r}_3 + \eta^{1/2} \sqrt{2C}~\mathbf{w}^{(k)}_1
	- C \eta^{3/2} \mathbf{M}^{-1} \sqrt{2C}~\left(\mathbf{w}^{(k)}_1/2 + \mathbf{w}^{(k)}_2 \right) \\
	&\quad + \eta^{5/2} \sum_{j=1}^n \left[ 
		\sum_{i=1}^n \left(\mathbf{M}^{-1} \sqrt{2C}~\mathbf{e_j} \right)^i 
			\frac{\partial}{\partial \theta^i}(-\nabla U(\boldsymbol{\theta}_3))
	\right] \mathbf{w}^{(k)}_{1,j} / 6  \\
	&\quad + \eta^{5/2} C^2 \mathbf{M}^{-2} \sqrt{2C}~\mathbf{w}^{(k)}_1 / 6
\end{split}
\end{equation}




==> quasisymapp_old.tex <==
We start our discussion by considering the fact that the evolution of a (deterministic) Hamiltonian \ode happens on a manifold with a structure that preserves the volume in the phase space, that is a symplectic manifolds.
\begin{definition}\label{definition:s_ode}
Any mapping 
$\boldsymbol{\kappa}:(p,q)\rightarrow (P,Q)$ is said to be symplectic if, and only if,
\begin{equation}\label{qssym}
    dP\wedge dQ=dp\wedge dq.
\end{equation}
The evolution of Hamiltonian \ode naturally respects this condition, as well as many other. 
\end{definition}
\maurizio{what do we mean with ``many other''?}\\
\dimitris{what does the wedge mean?}\\
\dimitris{maybe a gentle verbal (ans short) introduction of the different between symplectic, conformally symplectic, quasi-symplectic?}


The concept can be extended also to Hamiltonian \sde. When we consider quadratic potential for the momentum, $\frac{1}{2}||\boldsymbol{r}||^2$, it is possible to prove that the \sde of interest is conformally symplectic, as defined hereafter.
\begin{definition}\label{definition:qs_mapping}
Consider a generic (stochastic) mapping $\boldsymbol{\tau}:(p,q)\rightarrow (P,Q)$. We say that it is conformally symplectic (with constant $\gamma$) if, and only if,
\begin{equation}\label{qssym}
    dP\wedge dQ=\exp(-\gamma) dp\wedge dq
\end{equation}
\maurizio{Isn't it weird to call the Jacobian $\mathbf{Omega}$ instead of $\mathbf{J}$?}

Equivalently, the property \eqref{qssym} can be translated into
\begin{equation}
    \mathbf{\Omega}^\top\mathbf{J}\mathbf{\Omega}=\exp(-\gamma)\mathbf{J}
\end{equation}
where $\mathbf{\Omega}_{m,n}=\frac{\partial \tau_m(z)}{\partial z_n}$ is the (random) Jacobian and $\mathbf{J}=\begin{bmatrix}\mathbf{0}&-\mathbf{I}\\ \mathbf{I} &\mathbf{0}
\end{bmatrix}$. The mapping is said to be symplectic when it is conformally symplectic with $\gamma=0$.
\end{definition}

The fundamental result of interest discussed in this Section is reported in the following Theorem, which states that the stochastic evolution of any process described by eq.~\eqref{hamsde} contracts the volume exponentially in time.

\begin{theorem}\label{theorem:qssde}
Consider an Hamiltonian \sde of the form \eqref{hamsde} with $T(\boldsymbol{r})=\frac{1}{2}||\mathbf{M}^{-1}\boldsymbol{r}||^2$. 
Consider the stochastic evolution induced by this equation starting from generic initial conditions, i.e., $\zvect(t)=\mathbf{\tau}(\zvect(0))$.
Then $\tau$ is contracts the volume exponentially in time as $\det\left(\mathbf{\Omega}\right)=\exp\left(-C\mathrm{Tr}\left(\mathbf{M}^{-1}\right)t\right)$. 

Additionally, if $\mathbf{M}^{-1}=m\eye$ for some $m>0$ then the mapping is conformally symplectic with constant $Cm$.
\end{theorem}


\begin{proof}
We start from the generic case that the mapping is quasi-symplectic. 
Starting from eq.~\eqref{hamsde}, we have
\begin{equation}
    \dzvect^\top(t)=\nabla^\top H(\zvect(t))\begin{bmatrix} -\Cfrict & -\eye\\ \eye & \zerovect \end{bmatrix}^\top dt+\mathbf{dw}^\top(t)\begin{bmatrix} \sqrt{2\Cfrict} & \zerovect\\ \zerovect & \zerovect \end{bmatrix}
\end{equation}
Consequently,
\begin{flalign*}
   d\nabla_{\zvect(0)}\zvect^\top(t) & = \nabla_{\zvect(0)}\dzvect^\top(t)=\nabla_{\zvect(0)}\nabla^\top H(\zvect(t))\begin{bmatrix} -\Cfrict & -\eye\\ \eye & \zerovect \end{bmatrix}^\top dt+\nabla_{\zvect(0)}\mathbf{dw}^\top(t)\begin{bmatrix} \sqrt{2\Cfrict} & \zerovect\\ \zerovect & \zerovect \end{bmatrix} \\
   & = \nabla_{\zvect(0)}\nabla^\top H(\zvect(t))\begin{bmatrix} -\Cfrict & -\eye\\ \eye & \zerovect \end{bmatrix}^\top dt=\nabla_{\zvect(0)}\zvect^\top(t)\Delta H(\zvect(t))\begin{bmatrix} -\Cfrict & -\eye\\ \eye & \zerovect \end{bmatrix}^\top dt
\end{flalign*}
which can be rewritten as
\begin{equation*}
    \mathbf{d\Omega}^\top(t)=\mathbf{\Omega}^\top(t)\begin{bmatrix} \mathbf{M}^{-1} & \zerovect \\ \zerovect & \Delta_{\thetavect}U(\thetavect(t)) \end{bmatrix}\begin{bmatrix} -\Cfrict & -\eye\\ \eye & \zerovect \end{bmatrix}^\top dt.
\end{equation*}


By the rule of differentiation of determinants, we can write
\begin{flalign*}
  &d\det(\mathbf{\Omega}^\top(t))=\mathrm{Tr}\left(\mathrm{adj}\left(\mathbf{\Omega}^\top(t)\right) \mathbf{d\Omega}^\top(t)\right)=\\& \mathrm{Tr}\left(\mathrm{adj}\left(\mathbf{\Omega}^\top(t)\right) \mathbf{\Omega}^\top(t)\begin{bmatrix} \mathbf{M}^{-1} & \zerovect \\ \zerovect & \Delta_{\thetavect}U(\thetavect(t)) \end{bmatrix}\begin{bmatrix} -\Cfrict & -\eye\\ \eye & \zerovect \end{bmatrix}^\top dt\right)=\\
  &\det(\mathbf{\Omega}^\top(t))\mathrm{Tr}\left(\begin{bmatrix} \mathbf{M}^{-1} & \zerovect \\ \zerovect & \Delta_{\thetavect}U(\thetavect(t)) \end{bmatrix}\begin{bmatrix} -\Cfrict & -\eye\\ \eye & \zerovect \end{bmatrix}^\top dt\right)=\\
  &\det(\mathbf{\Omega}^\top(t))\mathrm{Tr}\left(\begin{bmatrix} \mathbf{M}^{-1} & \zerovect \\ \zerovect & \Delta_{\thetavect}U(\thetavect(t)) \end{bmatrix}\begin{bmatrix} -\Cfrict & \zerovect\\ \zerovect & \zerovect \end{bmatrix}^\top dt\right)=-\det(\mathbf{\Omega}^\top(t))C\mathrm{Tr}\left(\mathbf{M}^{-1}\right) dt.
\end{flalign*}
This, toghether with the condition $\mathbf{\Omega}(0)=\eye$ proves that
\begin{equation*}
   \det(\mathbf{\Omega}^\top(t))=\exp( -C\mathrm{Tr}\left(\mathbf{M}^{-1}\right)t)
\end{equation*}

\end{proof}


\dimitris{I introduced the proof environment for Theorem 4; is this ok?}\\
\dimitris{what is the next proof about?}\\

We then prove that whenever $\mathbf{M}^{-1}=m\eye$ the system is conformally symplectic.
Define $\mathbf{K}=\begin{bmatrix} -\Cfrict & \zerovect\\ \zerovect & \zerovect \end{bmatrix}, \mathbf{U}=\begin{bmatrix} m\eye & \zerovect \\ \zerovect & \Delta_{\thetavect}U(\thetavect(t)) \end{bmatrix} $ and then expand the following quantity 
\begin{flalign*}
 d(\mathbf{\Omega}^\top\mathbf{J}\mathbf{\Omega}) & = \mathbf{d\Omega}^\top\mathbf{J}\mathbf{\Omega}+\mathbf{\Omega}^\top\mathbf{J}\mathbf{d\Omega} \\
 & = \mathbf{\Omega}^\top\mathbf{U}(\mathbf{K}+\mathbf{J}^\top)\mathbf{J}\mathbf{\Omega}+\mathbf{\Omega}^\top\mathbf{J}(\mathbf{K}+\mathbf{J})\mathbf{U}\mathbf{\Omega}=\mathbf{\Omega}^\top\mathbf{U}\mathbf{K}\mathbf{J}\mathbf{\Omega}+\mathbf{\Omega}^\top\mathbf{J}\mathbf{K}\mathbf{U}\mathbf{\Omega}
\end{flalign*}
obtained considering $\mathbf{J}\mathbf{J}^\top=\eye,\mathbf{J}\mathbf{J}=-\eye$.
Since $\mathbf{K}\mathbf{U}=\begin{bmatrix} -C m\eye& \zerovect\\ \zerovect & \zerovect \end{bmatrix}$ we have consequently $\mathbf{K}\mathbf{U}=\mathbf{U}\mathbf{K}$.

Simple manipulations allow us to write 
\begin{flalign*}
   \mathbf{\Omega}^\top\mathbf{U}\mathbf{K}\mathbf{J}\mathbf{\Omega}+\mathbf{\Omega}^\top\mathbf{J}\mathbf{K}\mathbf{U}\mathbf{\Omega}=-Cm\mathbf{\Omega}^\top\mathbf{J}\mathbf{\Omega}
\end{flalign*}
Consequently, we have
\begin{flalign*}
  \mathbf{\Omega}^\top\mathbf{J}\mathbf{\Omega}=\exp(-Cmt)\mathbf{J}
\end{flalign*}



Finally, we are ready to introduce the concept of quasi-symplectic integrators as numerical schemes that aim at preserving the underlying geometry.
The precise definition is in the following.

\maurizio{maybe leave out the indices from the bold}
\begin{definition}\label{definition:qsintegrator}
  An numerical (stochastic) integrator $\phi: \mathbf{z_i}\rightarrow \mathbf{z_{i+1}}$ with step size $\eta$ is defined to be quasi-symplectic if the following two properties holds:
\begin{enumerate}
    \item The determinant of the Jacobian  $\mathbf{\Omega}=(\nabla_{\mathbf{z_{i-1}}}\phi(\mathbf{z_i})^\top)$ of the numerical integrator does not depend on $\mathbf{z_i}=(\mathbf{r_i},\boldsymbol{\theta_i})$
    \item In the limit of vanishing friction, i.e. $C \rightarrow 0$, the Jacobian $\mathbf{\Omega}$ satisfies the symplectic condition
    \begin{equation}
            \mathbf{\Omega}^\top\mathbf{J}\mathbf{\Omega}=\mathbf{J}
    \end{equation}
\end{enumerate}
Furhermore, if the following holds
\begin{equation}
    \mathbf{\Omega}^\top\mathbf{J}\mathbf{\Omega}=\exp(-C\eta)\mathbf{J},
\end{equation}

and consequently both aforementioned properties hold, the integrator is said to be conformally symplectic.
We notice that being conformally symplectic implies the quasi-symplectic condition.
\end{definition}


In the experimental section we analyzed the performance of different integration schemes (both quasi-symplectic and not) and clearly show that quasi-symplectic methods outperform non quasi-symplectic ones.
Among the quasi-symplectic class, we test Leapfrog, symmetric, Lie-Trotter (provided symplectic Hamiltonian integrator \maurizio{I don't get this text in parenthesis}) schemes.
As far as non quasi-symplectic schemes, we test the \euler and \rktwo ones.


==> related_work.tex <==
sThe stochastic processes described by \sdes have been intensively studied \cite{kloeden2013numerical,debussche2012weak}, with some of the authors putting a particular emphasis on the stationary property of these processes \cite{abdulle2014high,MILSTEIN200781}. In this work, as in \cite{abdulle2014high,abdulle2015long}, we are interested in the asymptotic (in time) performance of such sampling schemes. The reader is referred to \cite{vollmer2016exploration}, \cite{gao2018global},\cite{gao2018breaking},\cite{futami2020accelerating} \cite{xu2018global} for additional insights into the non asymptotic behaviour of the sampling methods. 

%General \sgmcmc stuff that has been used in the past to collect samples from the posterior \cite{welling2011bayesian} \cite{chen2014stochastic}
%\cite{ahn2012bayesian} \cite{Zhang2020Cyclical}. Even before that, \hmc was used \cite{neal2011mcmc} \cite{shahbaba2014split}.

We are interested in the symplectic geometry of Hamiltonian systems. Symplectic \citep{milstein2002symplectic} and quasi symplectic \citep{milstein2003quasi,abdulle2014high,bou2010long} \sdes have been studied in the past, albeit in a different context than Bayesian sampling. Recently, symplectic geometry has been revisited, to characterize generic optimization problems \cite{betancourt2018symplectic,francca2020conformal,francca2021dissipative}, whereas in this work we are intersted only on sampling properties.

As most of the recent literature, we study scalable methods considering data subsampling. Our methods are rooted in the geometrical view of splitting schemes for high dimensional Hamiltonian systems \cite{childs2019theory},\cite{suzuki1977convergence},\cite{hatano2005finding},\cite{childs2019nearly},\cite{low2019well}. Particularly relevant to the approach we propose in this paper are the works that explore randomized splitting schemes \cite{childs2019faster}, \cite{zhang2012randomized}. Earlier attempts \cite{pmlr-v37-betancourt15,shahbaba2014split} to use operator splitting as a tool to describe mini-batching focus on \hmc, whereas \sghmc and related schemes have never been studied, to the best of our knowledge, under this formalism.


==> tables/summary_integrators.tex <==




\newcommand{\updateEULER}{
\parbox{0.1\textwidth}{
\begin{align*}
\boldsymbol{\theta}_{i}&=\boldsymbol{\theta}_{i-1}+\eta\mathbf{r}_{i-1}, \\
\mathbf{r}_{i}&=\mathbf{r}_{i-1}-\eta C\mathbf{r}_{i-1}-\eta \nabla U(\boldsymbol{\theta}_{i-1})+\sqrt{2C\eta}\mathbf{w}
\end{align*}
}
}



\newcommand{\updateRKTWO}{
\parbox{0.1\textwidth}{
\begin{align*}
\thetavect^* &= \thetavect_{i-1}+\eta\rvect_{i-1}, \\
   \rvect^*&=\rvect_{i-1}-\eta \nabla U(\thetavect_{i-1})-\eta C \rvect_{i-1}+\sqrt{2 C\eta}\mathbf{w}, \\
    \thetavect_{i}&=\thetavect_{i-1}+\nicefrac{\eta}{2}\left(\rvect_{i-1}+\rvect^*\right),\\
    \rvect_i&=\rvect_{i-1}+\nicefrac{\eta}{2}\left(- \nabla U(\thetavect_{i-1})-C \rvect_{i-1}- \nabla U(\thetavect^*)-C \rvect^*\right)+\sqrt{2 C\eta}\mathbf{w}
\end{align*}
}
}


\newcommand{\updateLP}{
\parbox{0.1\textwidth}{
\begin{align*}
    \thetavect^*&=\thetavect_{i-1}+\nicefrac{\eta}{2}\rvect_{i-1}, \\
    \rvect_{i}&=\rvect_{i-1}-\eta \nabla U(\thetavect^*)-\eta C \rvect_{i-1}+\sqrt{2 C\eta}\mathbf{w}, \\
    \thetavect_{i}&=\thetavect^*+\nicefrac{\eta}{2}\rvect_{i}.
\end{align*}
}
}


\newcommand{\updateLT}{
\parbox{0.1\textwidth}{
\begin{align*}
\rvect^* &= \rvect_{i-1}-\nicefrac{\eta}{2} \nabla U(\thetavect_{i-1}),\\
\thetavect_i &= \thetavect_{i-1}+\eta\rvect^*,\rvect^{'}=\rvect^*-\nicefrac{\eta}{2} \nabla U(\thetavect_{i}),\\
\mathbf{r}_i &= e^{-C\eta}\mathbf{r}^{'}+\sqrt{1-e^{-2Ct}}\mathbf{w}
\end{align*}
}
}

    

%\boldsymbol{\theta}_{i}=\boldsymbol{\theta}_{i-1}+\eta\mathbf{r}_{i-1},
%\mathbf{r}_{i}=\mathbf{r}_{i-1}-\eta C\mathbf{r}_{i-1}-\eta \nabla U(\boldsymbol{\theta}_{i-1})+\sqrt{2C\eta}\mathbf{w}, \mathbf{w}\sim \mathcal{N}(\zerovect,\eye)


\begin{tabular}{l|l|lc}
    \toprule
    Name            & Update rule       & Order                 & Symplectic \\
    \hline
    \hline
    %\euler          & \updateEULER      & $\mathcal{O}(\eta)$  & No          \\
    %\hline
    \rktwo          & \updateRKTWO      & $\mathcal{O}(\eta^2)$ & No         \\
    \hline
    \leapfrog       & \updateLP         & $\mathcal{O}(\eta)$   & Yes        \\
    \hline
    \lietrotter     & \updateLT         & $\mathcal{O}(\eta^2)$ & Yes        \\
    \bottomrule
\end{tabular}


==> tables/summary_integrators_reshape.tex <==




\newcommand{\updateEULER}{
\parbox{0.1\textwidth}{
\begin{align*}
\boldsymbol{\theta}_{i}&=\boldsymbol{\theta}_{i-1}+\eta\mathbf{r}_{i-1}, \\
\mathbf{r}_{i}&=\mathbf{r}_{i-1}-\eta C\mathbf{r}_{i-1}-\eta \nabla U(\boldsymbol{\theta}_{i-1})+\sqrt{2C\eta}\mathbf{w}
\end{align*}
}
}



\newcommand{\updateRKTWO}{
\parbox{0.1\textwidth}{
\begin{align*}
\thetavect^* &= \thetavect_{i-1}+\eta\rvect_{i-1}, \\
   \rvect^*&=\rvect_{i-1}-\eta \nabla U(\thetavect_{i-1})-\eta C \rvect_{i-1}+\sqrt{2 C\eta}\mathbf{w}, \\
    \thetavect_{i}&=\thetavect_{i-1}+\nicefrac{\eta}{2}\left(\rvect_{i-1}+\rvect^*\right),\\
    \rvect_i&=\rvect_{i-1}+\\\nicefrac{\eta}{2}&\left(- \nabla U(\thetavect_{i-1})-C \rvect_{i-1}- \nabla U(\thetavect^*)-C \rvect^*\right)+\sqrt{2 C\eta}\mathbf{w}
\end{align*}
}
}


\newcommand{\updateLP}{
\parbox{0.1\textwidth}{
\begin{align*}
    \thetavect^*&=\thetavect_{i-1}+\nicefrac{\eta}{2}\rvect_{i-1}, \\
    \rvect_{i}&=\rvect_{i-1}-\eta \nabla U(\thetavect^*)-\eta C \rvect_{i-1}+\sqrt{2 C\eta}\mathbf{w}, \\
    \thetavect_{i}&=\thetavect^*+\nicefrac{\eta}{2}\rvect_{i}.
\end{align*}
}
}


\newcommand{\updateLT}{
\parbox{0.1\textwidth}{
\begin{align*}
\rvect^* &= \rvect_{i-1}-\nicefrac{\eta}{2} \nabla U(\thetavect_{i-1}),\\
\thetavect_i &= \thetavect_{i-1}+\eta\rvect^*,\rvect^{'}=\rvect^*-\nicefrac{\eta}{2} \nabla U(\thetavect_{i}),\\
\mathbf{r}_i &= e^{-C\eta}\mathbf{r}^{'}+\sqrt{1-e^{-2Ct}}\mathbf{w}
\end{align*}
}
}

    

%\boldsymbol{\theta}_{i}=\boldsymbol{\theta}_{i-1}+\eta\mathbf{r}_{i-1},
%\mathbf{r}_{i}=\mathbf{r}_{i-1}-\eta C\mathbf{r}_{i-1}-\eta \nabla U(\boldsymbol{\theta}_{i-1})+\sqrt{2C\eta}\mathbf{w}, \mathbf{w}\sim \mathcal{N}(\zerovect,\eye)


\begin{tabular}{l|l|l|l}\toprule
      &  \rktwo & \leapfrog & \lietrotter\\\hline
      & \updateRKTWO & \updateLP & \updateLT\\
     \bottomrule
\end{tabular}



==> tables/summary_integrators_short.tex <==




\newcommand{\updateEULER}{
\parbox{0.1\textwidth}{
\begin{align*}
\boldsymbol{\theta}_{i}&=\boldsymbol{\theta}_{i-1}+\eta\mathbf{r}_{i-1}, \\
\mathbf{r}_{i}&=\mathbf{r}_{i-1}-\eta C\mathbf{r}_{i-1}-\eta \nabla U(\boldsymbol{\theta}_{i-1})+\sqrt{2C\eta}\mathbf{w}
\end{align*}
}
}



\newcommand{\updateRKTWO}{
\parbox{0.1\textwidth}{
\begin{align*}
\thetavect^* &= \thetavect_{i-1}+\eta\rvect_{i-1},
   \rvect^*=\rvect_{i-1}-\eta \nabla U(\thetavect_{i-1})-\eta C \rvect_{i-1}+\sqrt{2 C\eta}\mathbf{w}, \\
    \thetavect_{i}&=\thetavect_{i-1}+\nicefrac{\eta}{2}\left(\rvect_{i-1}+\rvect^*\right),\\
    \rvect_i&=\rvect_{i-1}+\nicefrac{\eta}{2}\left(- \nabla U(\thetavect_{i-1})-C \rvect_{i-1}- \nabla U(\thetavect^*)-C \rvect^*\right)+\sqrt{2 C\eta}\mathbf{w}
\end{align*}
}
}


\newcommand{\updateLP}{
\parbox{0.1\textwidth}{
\begin{align*}
    \thetavect^*&=\thetavect_{i-1}+\nicefrac{\eta}{2}\rvect_{i-1}, \quad
    \rvect_{i}=\rvect_{i-1}-\eta \nabla U(\thetavect^*)-\eta C \rvect_{i-1}+\sqrt{2 C\eta}\mathbf{w},\quad
    \thetavect_{i}=\thetavect^*+\nicefrac{\eta}{2}\rvect_{i}.
\end{align*}
}
}


\newcommand{\updateLT}{
\parbox{0.1\textwidth}{
\begin{align*}
\rvect^* &= \rvect_{i-1}-\nicefrac{\eta}{2} \nabla U(\thetavect_{i-1}),\\
\thetavect_i &= \thetavect_{i-1}+\eta\rvect^*,\rvect^{'}=\rvect^*-\nicefrac{\eta}{2} \nabla U(\thetavect_{i}), \quad
\mathbf{r}_i = e^{-C\eta}\mathbf{r}^{'}+\sqrt{1-e^{-2Ct}}\mathbf{w}
\end{align*}
}
}

    

%\boldsymbol{\theta}_{i}=\boldsymbol{\theta}_{i-1}+\eta\mathbf{r}_{i-1},
%\mathbf{r}_{i}=\mathbf{r}_{i-1}-\eta C\mathbf{r}_{i-1}-\eta \nabla U(\boldsymbol{\theta}_{i-1})+\sqrt{2C\eta}\mathbf{w}, \mathbf{w}\sim \mathcal{N}(\zerovect,\eye)


\begin{tabular}{l|l|lc}
    \toprule
    Name            & Update rule       & Order                 & Symplectic \\
    \hline
    \hline
    %\euler          & \updateEULER      & $\mathcal{O}(\eta)$  & No          \\
    %\hline
    \rktwo          & \updateRKTWO      & $\mathcal{O}(\eta^2)$ & No         \\
    \hline
    \leapfrog       & \updateLP         & $\mathcal{O}(\eta)$   & Yes        \\
    \hline
    \lietrotter {\color{red} We have to split r for the new thm}    & \updateLT         & $\mathcal{O}(\eta^2)$ & Yes        \\
    \bottomrule
\end{tabular}

